Text Data Augmentation for Large Language Models: A Comprehensive Survey of Methods, Challenges, and Opportunities

The increasing size and complexity of pre-trained language models have demonstrated superior performance in many applications, but they usually require large training datasets to be adequately trained. Insufficient training sets could unexpectedly make the model overfit and fail to cope with complex tasks. Large language models (LLMs) trained on extensive corpora have prominent text generation capabilities, which improve the quality and quantity of data and play a crucial role in data augmentation. Specifically, distinctive prompt templates are given in personalised tasks to guide LLMs in generating the required content. Recent promising retrieval-based techniques further improve the expressive performance of LLMs in data augmentation by introducing external knowledge to enable them to produce more grounded-truth data. This survey provides an in-depth analysis of data augmentation in LLMs, classifying the techniques into Simple Augmentation, Prompt-based Augmentation, Retrieval-based Augmentation and Hybrid Augmentation. We summarise the post-processing approaches in data augmentation, which contributes significantly to refining the augmented data and enabling the model to filter out unfaithful content. Then, we provide the common tasks and evaluation metrics. Finally, we introduce existing challenges and future opportunities that could bring further improvement to data augmentation.

==> Table/Demonstration.tex <==
	\begin{table*}[h]
				\caption{A demonstration for each prompt-based method.}
          \scalebox{0.8}{  
		\begin{tabular}{llll}
	 				
\toprule

Prompt Complexity                     & Prompt-based Methods       & Demonstrations                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     &  \\
\midrule
                                      & Cloze Prompting            & \textbf{\textcolor{red}{[M]}}
 use machine learning \textbf{\textcolor{red}{[M]}} AI techniques \textbf{\textcolor{red}{[M]}}                                                                                                               &  \\
 \cline{2-3}  
   \multirow{-3}{*}{Single-step Prompts}  & Zero-shot Prompting        & \begin{tabular}[c]{@{}l@{}}Dataset: SST-2\\ Class: Positive\\ Prompt: Generate 20 sentences that are positive reviews to a movie\\ Class: Negative\\ Prompt: Generate 20 sentences that are negative reviews to a movie\end{tabular}                                                                                                                                                    &  \\
\cline{2-3}   
 & Few-shot Prompting         & \begin{tabular}[c]{@{}l@{}}Input Prompt: The following sentences belong to the same category music likeness:\\ Example 1: i like soft rock music\\ Example 2: current song rating three stars\\ . . . . . .\\ Example 9: the song in background is cool\\ Example 10: i am the living blues\\ Example 11:\end{tabular}                                                                                                                                                                                                                                                                                                                             &  \\

\hline
Multi-steps Prompts                   & Chain-of-Thought Prompting & \begin{tabular}[c]{@{}l@{}}Chain of Thought\\ 1. Identify the predicates of given text.\\ 2. Centered on the predicate, rewrite the given text word-by-word.\\ 3. The order of that change of words is not allowed.\end{tabular}                                                                                                                                                                                                                                                                                                                                                                                                                   &  \\
\hline
                                      & Role Prompting             & \begin{tabular}[c]{@{}l@{}}The following is a conversation with an AI assistant. The assistant is helpful, \\ empathetic, clever, and very friendly. It can use various support skills to \\ provide emotional support to human.\\ Human: I moved into a new state recently, and there’s a lot to do, but I don't \\ have any friends in the new place I stay at.\\ AI:\end{tabular}                                                                                                                                                                                                                                                               &  \\

    \cline{2-3}  
                                      & Tuple Prompting            & \begin{tabular}[c]{@{}l@{}}An LM-based taskoriented dialogue system can be considered as \textbf{\textcolor{red}{tuples (c, b, d, r)}}, \\ where r is the system's response, c is the context (i.e., a concatenation of all previous \\ utterances in the dialogue – both system's and user's), b is the system's belief state \\ which is also used for querying the database, and d are the database results.\end{tabular}                                                      &  \\
\cline{2-3}  
   \multirow{-4}{*}{Structured Prompts}                                    & Concatenation Prompting    & \begin{tabular}[c]{@{}l@{}}x = \textless S \textgreater \textbf{\textcolor{red}{[demo]}} Demonstration \textbf{\textcolor{red}{[demo]}} Question \textbf{\textcolor{red}{[sep]}} Input Context \textless /S \textgreater\\ we add three new tokens: {[}demo{]}, {[}tgr{]} and {[}sep\_arg{]}. \\ More specifically, {[}demo{]} denotes which part of the input sequence is the demonstration, \\ {[}trg{]} marks the trigger of the event in the input context, {[}sep\_arg{]} is used as the \\ separator token gold arguments.\end{tabular}                                                    &  \\
\cline{2-3}  
 & Template Prompting         & \begin{tabular}[c]{@{}l@{}}Given a sentence: """ \{sentence\} """ Given entities in above sentence separated \\ by comma: """ \{entities\} """\\ Please generate 5 new sentences using \{new context\}. In each new sentence, use each\\ given entity exactly once, keep their entity type in the given sentence, introduce\\ no other entities. \\ Desired format: \\ Kept Entities: \textless{}all kept entities separated by comma\textgreater New sentence: \textless{}new sentence\textgreater \\ Kept Entities: \textless{}all kept entities separated by comma\textgreater New sentence: \textless{}new sentence\textgreater{}\end{tabular} &    \\
					\bottomrule
				\end{tabular}
		}		
				\label{tap:prompt-examples}
			\end{table*}                           
			
			

==> Table/LLMsinDA.tex <==

	\begin{table*}[h]
		\caption{LLMs in DA.}
		\centering
		% \begin{tabularx}{\textwidth}{lYY|lYY|lYY}
			%\begin{tabular}{p{2.5cm}p{1cm}p{2.5cm}|p{2.5cm}p{1cm}p{2.5cm}|p{2.5cm}p{1cm}p{2.5cm}}
			\begin{tabular}{ccp{2.3cm}ccp{2.3cm}ccp{2.3cm}}     
				
				\toprule
				Encoder-only    & Params & Method    & Decoder-only       & Params & Method                                 & Encoder-decoder & Params & Method \\
				\midrule
				\cellcolor[HTML]{F9CBAA}ALBERT Base & \cellcolor[HTML]{F9CBAA}11M & \cite{FlipDA} & \cellcolor[HTML]{D0E4F6}GPT-2 Small & \cellcolor[HTML]{D0E4F6}117M & \cite{TransformersDA},\cite{Human-in-the-loop} & T5 Small & 60M & \\
				
				ALBERT Large & 17M &  & GPT-2 Medium & 345M &  & FLAN-T5 Small & 60M & \\
				
				ALBERT XLarge & 58M &  & \cellcolor[HTML]{D0E4F6}GPT-3(Ada) & \cellcolor[HTML]{D0E4F6}350M & \cite{GPT3Mix},\cite{DA-intent} & BART Base & 140M & \\
				
				\cellcolor[HTML]{F9CBAA}DistilBERT Base & \cellcolor[HTML]{F9CBAA}66M & \cite{GPT3Mix},\cite{PROMPTING},\cite{PromptMix},\cite{GENIUS} & GPT-2 Large & 774M & & \cellcolor[HTML]{D0E4F6}T5 Base & \cellcolor[HTML]{D0E4F6}220M & \cite{DAGAM},\cite{Generative-DA} \\
				
				\cellcolor[HTML]{F9CBAA}DeBERTa Base & \cellcolor[HTML]{F9CBAA}100M & \cite{FlipDA} & \cellcolor[HTML]{D0E4F6}GPT-3(Babbage) & \cellcolor[HTML]{D0E4F6}1.3B & \cite{GPT3Mix},\cite{DA-intent}& \cellcolor[HTML]{F9CBAA}FLAN-T5 Base & \cellcolor[HTML]{F9CBAA}220M & \cite{ICLEF} \\
				
				\multicolumn{1}{c}{\cellcolor[HTML]{F9CBAA}}                            & \multicolumn{1}{c}{\cellcolor[HTML]{F9CBAA}}                       &                                                                                                                                   & \multicolumn{1}{c}{\cellcolor[HTML]{D0E4F6}}                               & \multicolumn{1}{c}{\cellcolor[HTML]{D0E4F6}}                       & \multicolumn{1}{c}{}                            & \multicolumn{1}{c}{}                         & \multicolumn{1}{c}{}                       & \multicolumn{1}{c}{}                   \\
				\multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor[HTML]{F9CBAA}BERT Base}} & \multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor[HTML]{F9CBAA}110M}} & \multirow{-2}{*}{\begin{tabular}[c]{@{}l@{}}\cite{TransformersDA},\cite{GPT3Mix},\cite{DAGAM},\cite{AugGPT},\\ \cite{ZeroShotDataAug},\cite{HiPSTG},\cite{LLM-DA},\cite{PromptMix}\end{tabular}} & \multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor[HTML]{D0E4F6}GPT-2 XLarge}} & \multicolumn{1}{c}{\multirow{-2}{*}{\cellcolor[HTML]{D0E4F6}1.5B}} & \multicolumn{1}{c}{\multirow{-2}{*}{\cite{PROMPTING}}} & \multicolumn{1}{c}{\multirow{-2}{*}{monoT5}} & \multicolumn{1}{c}{\multirow{-2}{*}{220M}} & \multicolumn{1}{c}{\multirow{-2}{*}{}}\\
				
				
				\cellcolor[HTML]{F9CBAA}ClinicalBERT & \cellcolor[HTML]{F9CBAA}110M & \cite{Healthcare-DA} & \cellcolor[HTML]{D0E4F6}GPT-J & \cellcolor[HTML]{D0E4F6}6B & \cite{AugESC},\cite{Prefix-Prompt} & \cellcolor[HTML]{F9CBAA}BART Large & \cellcolor[HTML]{F9CBAA}400M & \cite{Synthetic-DA}\\
				
				\cellcolor[HTML]{F9CBAA}mBERT & \cellcolor[HTML]{F9CBAA}110M & \cite{LLM-powered} & \cellcolor[HTML]{D0E4F6}GPT-3(Curie) & \cellcolor[HTML]{D0E4F6}6.7B & \cite{Prefix-Prompt},\cite{GPT3Mix},\cite{DA-intent},\cite{WANLI}& \cellcolor[HTML]{F9CBAA}mBART-50 & \cellcolor[HTML]{F9CBAA}610M & \cite{DA-NMT}\\
				
				\cellcolor[HTML]{F9CBAA}RoBERTa Base & \cellcolor[HTML]{F9CBAA}125M & \cite{Read-Com},\cite{Generative-DA},\cite{LLM-DA} & \cellcolor[HTML]{D0E4F6}Qwen & \cellcolor[HTML]{D0E4F6}7B & \cite{LLM–Assisted} & \cellcolor[HTML]{D0E4F6}T5 Large & \cellcolor[HTML]{D0E4F6}770M & \cite{FlipDA}\\
				
				ALBERT XXLarge & 223M & & \cellcolor[HTML]{D0E4F6}MPT & \cellcolor[HTML]{D0E4F6}7B & \cite{ICLEF}& \cellcolor[HTML]{F9CBAA}FLAN-T5 Large & \cellcolor[HTML]{F9CBAA}770M & \cite{Dialogue-Convert} \\
				
				\cellcolor[HTML]{F9CBAA}XLM-R Base & \cellcolor[HTML]{F9CBAA}250M & \cite{LLM-powered} & \cellcolor[HTML]{D0E4F6}LLAMA & \cellcolor[HTML]{D0E4F6}7B & \cite{ICLEF},\cite{LLM2LLM} & PaLM 2 Small & 800M & \\
				
				\cellcolor[HTML]{F9CBAA}BERT Large & \cellcolor[HTML]{F9CBAA}340M & \cite{DA-intent} & StableVicuna & 7B & & PaLM 2 Medium & 2.7B & \\
				
				DeBERTa Large & 350M & & Vicuna & 7B & & T5 3B & 3B & \\
				
				\cellcolor[HTML]{F9CBAA}RoBERTa Large & \cellcolor[HTML]{F9CBAA}355M & \cite{WANLI},\cite{Synthetic-DA},\cite{GENIUS} & \cellcolor[HTML]{D0E4F6}Dolly-v2 & \cellcolor[HTML]{D0E4F6}12B & \cite{Human-in-the-loop} & \cellcolor[HTML]{F9CBAA}FLAN-T5 XL & \cellcolor[HTML]{F9CBAA}3B & \cite{Dialogue-Convert} \\
				
				\cellcolor[HTML]{F9CBAA}XLM-R Large & \cellcolor[HTML]{F9CBAA}560M & \cite{LLM-powered} & \cellcolor[HTML]{D0E4F6}LLAMA & \cellcolor[HTML]{D0E4F6}13B & \cite{Dialogue-Convert} & PaLM 2 Large & 8B & \\
				
				& & & \cellcolor[HTML]{D0E4F6}Vicuna & \cellcolor[HTML]{D0E4F6}13B & \cite{ICLEF}& \cellcolor[HTML]{F9CBAA}T5 11B & \cellcolor[HTML]{F9CBAA}11B & \cite{Unnatural-instructions} \\
				
				& & & \cellcolor[HTML]{D0E4F6}StableVicuna & \cellcolor[HTML]{D0E4F6}13B &\cite{LLM-powered} & \cellcolor[HTML]{F9CBAA}FLAN-T5 XXL & \cellcolor[HTML]{F9CBAA}11B & \cite{Dialogue-Convert}\\
				
				& & & \cellcolor[HTML]{D0E4F6}Tülu & \cellcolor[HTML]{D0E4F6}13B & \cite{ICLEF}& PaLM 2 XL & 16B & \\
				
				& & & \cellcolor[HTML]{D0E4F6}GPT-NeoX & \cellcolor[HTML]{D0E4F6}20B & \cite{Synthetic-DA},\cite{Prefix-Prompt}& \cellcolor[HTML]{D0E4F6}PaLM2 & \cellcolor[HTML]{D0E4F6}540B & \cite{DAIL} \\
				
				& & & LLAMA 30B & 30B & & & & \\
				
				& & & \cellcolor[HTML]{D0E4F6}Falcon & \cellcolor[HTML]{D0E4F6}40B & \cite{ICLEF} & & & \\
				
				& & & LLAMA 
				
				65B & 65B & & & & \\
				
				& & & \cellcolor[HTML]{D0E4F6}LLaMA2 70B & \cellcolor[HTML]{D0E4F6}70B & \cite{PromptMix} & & & \\
				
				& & & \cellcolor[HTML]{D0E4F6}Airoboros-L2 & \cellcolor[HTML]{D0E4F6}70B & \cite{LLM2LLM} & & & \\
				
				& & & \cellcolor[HTML]{D0E4F6}GPT-3(Davinci) & \cellcolor[HTML]{D0E4F6}175B & \cite{Prefix-Prompt},\cite{GPT3Mix},\cite{DA-intent}& & & \\
				
				&  &  & \multicolumn{1}{c}{\cellcolor[HTML]{D0E4F6}}                          & \multicolumn{1}{c}{\cellcolor[HTML]{D0E4F6}}                      &                                                                                                                                                                                              &  &  &  \\
				&  &  & \multicolumn{1}{c}{\cellcolor[HTML]{D0E4F6}}                          & \multicolumn{1}{c}{\cellcolor[HTML]{D0E4F6}}                      &                                                                                                                                                                                              &  &  &  \\
				&  &  & \multicolumn{1}{c}{\multirow{-3}{*}{\cellcolor[HTML]{D0E4F6}GPT-3.5}} & \multicolumn{1}{c}{\multirow{-3}{*}{\cellcolor[HTML]{D0E4F6}NAN}} & \multirow{-3}{*}{\begin{tabular}[c]{@{}l@{}}\cite{AugGPT},\cite{DAIL},\cite{DA-NMT},\cite{EPA},\cite{ZeroShotDataAug},\\  \cite{Dialogue-Convert},\cite{LLM-powered},\cite{Healthcare-DA},\cite{ICLEF},\cite{LLM-DA},\\ \cite{LLM–Assisted},\cite{LLM2LLM},\cite{PromptMix}\end{tabular}} &  &  &  \\
				&  &  & \cellcolor[HTML]{D0E4F6}GPT-4                                         & \cellcolor[HTML]{D0E4F6}NAN                                       & \cite{Read-Com},\cite{LLM-powered}                                                                                                                                                                      &  &  & \\
				\bottomrule
			\end{tabular}
			
			\label{tab:LLMs}
		\end{table*}
		

==> Table/Reteieval-type.tex <==
		\begin{table*}[h]
						%  \begin{tabularx}{\textwidth}{YYYYYYY}
							\caption{Retrieval-based method, retriever type}
							\begin{tabular}{c c c c c c p{3.5cm}} 
								\toprule
								\multicolumn{1}{c}{Method}                  & \multicolumn{1}{c}{Prompt-based method}                & \multicolumn{1}{c}{Retrieval-based(hybrid) method}                                                   & \multicolumn{1}{c}{Retriever type}                         & \multicolumn{1}{c}{Retriever method}                                                              &  &  \\
								\midrule
								
								\multicolumn{5}{c}{Retrieval-based method}\\
								\hline
								\multicolumn{1}{c}{AugmentedSBERT} \cite{AugmentedSBERT}        & \multicolumn{1}{c}{-}                                      & \multicolumn{1}{c}{Incorporate data}                                                         & \multicolumn{1}{c}{Sparse retrieval}                       & \multicolumn{1}{c}{BM25}                                                                          &  &  \\ \cline{1-5}
								\multicolumn{1}{c}{zicl}  \cite{zicl}                 & \multicolumn{1}{c}{-}                                      & \multicolumn{1}{c}{Incorporate data}                                                         & \multicolumn{1}{c}{Dense retrieval}                        & \multicolumn{1}{c}{SimCSE}                                                                        &  &  \\ \cline{1-5}
								\multicolumn{1}{c}{\multirow{2}{*}{DAPDR}} \cite{DAPDR}  & \multicolumn{1}{c}{\multirow{2}{*}{-}}                     & \multicolumn{1}{c}{\multirow{2}{*}{Query generation}}                                        & \multicolumn{1}{c}{Dense retrieval}                        & \multicolumn{1}{c}{DPR, BERT, SBERT, MPNET}                                                       &  &  \\ \cline{4-5}
								\multicolumn{1}{c}{}                        & \multicolumn{1}{c}{}                                       & \multicolumn{1}{c}{}                                                                         & \multicolumn{1}{c}{Sparse retrieval}                       & \multicolumn{1}{c}{BM25}                                                                          &  &  \\ \cline{1-5}
								\hline
								\multicolumn{5}{c}{Hybrid method}\\
								\hline
								\multicolumn{1}{c}{InPars}    \cite{InPars}              & \multicolumn{1}{c}{Few-shot prompting}                     & \multicolumn{1}{c}{Query generation}                                                         & \multicolumn{1}{c}{Multi-stage retrieval}                  & \multicolumn{1}{c}{BM25 followed by a reranker monoT5}                               &  &  \\ \cline{1-5}
								\multicolumn{1}{c}{DAICL}   \cite{DAICL}                & \multicolumn{1}{c}{Few-shot prompting}                     & \multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}Incorporate data\\ Prepend data\end{tabular}} & \multicolumn{1}{c}{Dense retrieval}                        & \multicolumn{1}{c}{SimCSE, BERTScore}                                                             &  &  \\ \cline{1-5}
								\multicolumn{1}{c}{Promptagator}   \cite{Promptagator}         & \multicolumn{1}{c}{Few-shot prompting}                     & \multicolumn{1}{c}{Query generation}                                                         & \multicolumn{1}{c}{Dense retrieval}                        & \multicolumn{1}{c}{GTR}                                                                           &  &  \\ \cline{1-5}
								\multicolumn{1}{c}{KAPING}  \cite{KAPING}                & \multicolumn{1}{c}{Instruction-following}                  & \multicolumn{1}{c}{Knowledge injection}                                                      & \multicolumn{1}{c}{Dense retrieval}                        & \multicolumn{1}{c}{MPNet, TAS-B}                                                                  &  &  \\ \cline{1-5}
								\multicolumn{1}{c}{\multirow{2}{*}{UDAPDR}} \cite{UDAPDR} & \multicolumn{1}{c}{Few-shot prompting,}                    & \multicolumn{1}{c}{\multirow{2}{*}{Query generation}}                                        & \multicolumn{1}{c}{\multirow{2}{*}{Multi-stage retrieval}} & \multicolumn{1}{c}{\multirow{2}{*}{ColBERTv2 followed by a reranker DeBERTaV3}} &  &  \\ \cline{2-2}
								\multicolumn{1}{c}{}                        & \multicolumn{1}{c}{Zero-shot prompting}                    & \multicolumn{1}{c}{}                                                                         & \multicolumn{1}{c}{}                                       & \multicolumn{1}{c}{}                                                                              &  &  \\ \cline{1-5}
								\multicolumn{1}{c}{\multirow{2}{*}{ALCE}} \cite{ALCE}  & \multicolumn{1}{c}{\multirow{2}{*}{Instruction-following}} & \multicolumn{1}{c}{\multirow{2}{*}{Knowledge injection}}                                     & \multicolumn{1}{c}{Dense retrieval}                        & \multicolumn{1}{c}{GTR, DPR}                                                                      &  &  \\ \cline{4-5}
								\multicolumn{1}{c}{}                        & \multicolumn{1}{c}{}                                       & \multicolumn{1}{c}{}                                                                         & \multicolumn{1}{c}{Sparse retrieval}                       & \multicolumn{1}{c}{BM25}                                                                          &  &  \\ \cline{1-5}
								\multicolumn{1}{c}{RADA}   \cite{RADA}                 & \multicolumn{1}{c}{Instruction-following}                  & \multicolumn{1}{c}{Knowledge injection}                                                      & \multicolumn{1}{c}{Dense retrieval}                        & \multicolumn{1}{c}{DistilBert TAS-B}                                                              &  &  \\ 
								\bottomrule
								
							\end{tabular}
							\label{retrieval-type}
						\end{table*}
						
